Learning Neural PDE Solvers with Convergence Guarantees

Partial differential equations (PDEs) are widely used across the physical and computational sciences. Decades of research and engineering went into designing fast iterative solution methods. Existing solvers are general purpose, but may be sub-optimal for specific classes of problems. In contrast to existing hand-crafted solutions, we propose an approach to learn a fast iterative solver tailored to a specific domain. We achieve this goal by learning to modify the updates of an existing solver using a deep neural network. Crucially, our approach is proven to preserve strong correctness and convergence guarantees. After training on a single geometry, our model generalizes to a wide variety of geometries and boundary conditions, and achieves 2-3 times speedup compared to state-of-the-art solvers.

==> Sections/old.tex <==

\begin{proof}
Observe that

\begin{equation}
\label{eq:Phi}
\Phi(u) = Tu+b+H(Tu+b-u) = (T+HT-H)u+Hb+b
\end{equation}

From Thereom~\ref{thm:spectral_norm}, a valid $H$ should satisfy $\rho(T + HT - H) < 1$. Because the spectral norm $\rho$ is convex, and $T+HT-H$ is linear in $H$, so $\rho(T+HT-H)$ is convex in $H$ as well. Thus, the set of valid $H$ must be convex because it is a sub-level set of the convex function $\rho(T+HT-H)$.


%%%%%%%%%%%%%% Moved this part to Section 2.3 %%%%%%%%%%%%%%
% $u^*$ is a fixed point iff $u^*=(T+HT-H)u^*+Hb+b$, or equivalently $(I-T-HT+H)u^*=Hb+b$, and the fixed point is unique iff $I-T-HT+H$ is full rank. Let $\lambda_{\mathrm{min}}$ denote the smallest eigenvalue, we have
% \[ \lambda_{\mathrm{min}}(I-T-HT+H) \geq 1 - \rho(T+HT-H) \]
% Therefore the fixed point is unique if
% \[ \rho(T+HT-H) < 1 \] 
% We have shown that the correct solution is a fixed point. Therefore, under above condition
% \begin{itemize}
%     \item $\Psi$ converges to a stable fixed point from any initialization (if and only if)
%     \item Fixed point is unique (if)
%     \item Correct solution is a fixed point (always true)
% \end{itemize}
% Based on these observations we conclude that $H$ is valid iff $\rho(T+HT-H) < 1$. 

% Suppose $H_1, H_2$ are valid. Let $H=\alpha H_1 + (1-\alpha)H_2$, $0 \leq \alpha \leq 1$, then
% \begin{align*}
%     \rho(T+H(T-I)) &= \rho(T+(\alpha H_1 + (1-\alpha)H_2)(T-I)) \\
%     &= \rho(\alpha(T+H_1(T-I)) + (1 - \alpha)(T+H_2(T-I)) \\
%     &\leq \alpha \rho(T+H_1(T-I)) + (1-\alpha) \rho(T+H_2(T-I)) &  \mathrm{(by\ convexity\ of\ } \rho)  \\ 
%     &< \alpha + (1-\alpha) = 1
% \end{align*} 
% Therefore $H$ is also valid. This means that the set of valid $H$ is convex. 
To prove that it is open, observe that $\rho$ is a continuous function, so $\rho(T+H(T-I))$ is continuous in $H$. Therefore if $\rho(T+H(T-I)) < 1$, for any $C\in \mathbb{R}^{n\times n}$ with $\lVert C \rVert_2 \leq 1$,

\begin{equation}
\lim_{\epsilon \to 0} \rho(T+(H+\epsilon C)(T-I)) < 1  \mathrm {\ uniformly}
\end{equation}

This means that for sufficiently small $\epsilon$, $H+\epsilon C$ is valid for all $C$ such that $\lVert C \rVert_2 \leq 1$. Therefore, the set of valid $H$ is open under $\lVert \cdot \rVert_2$. In addition all norms are topologically equivalent in $\mathbb{R}^{n \times n}$ so the conclusion is independent of choice of norm.  % Because this function $<1$ for $B$, then it must be $<1$ for $B+\epsilon C$ if $\epsilon$ is sufficiently small. 

To prove the second part, we must first rewrite our equations to generalize to any geometry. Note that in the equations $Au = f$ and $Tu + b$, the matrices $A$ and $T$ depend on the geometry. We now extend the domain to an infinite or sufficiently large domain, and each point is either a boundary or a \todo{something}. Let $E$ be a diagonal matrix such that $E_{ii} = 1$ if point $i$ is a boundary, and 0 otherwise. Note that $E^2 = E$ and $E$ cannot be identity $I$. Thus, we rewrite $\Psi$ and $\Phi$, (Additionally require $Ec=0$)

\begin{equation}
\begin{aligned}
    \Psi(u) &= E(Tu + b) + c \\
    \Phi(u) &= E( \Psi(u) + H(\Psi(u) - u)) + c %&= (EHET + ET - EH)u + c'
\end{aligned}
\end{equation}
An alternative way to write the second expression is
\[ \Phi(u) = E(Tu+H(\Psi(u)-u)) + Eb + c \]
The matrix $E$ can be interpreted as masking out the boundary points, and $c$ represent the boundary values. Thus, $E$ represents the geometry of the domain. Given a valid $H$ on a specific geometry $E$.
To study the system we define an auxiliary variable $w_{t+1} = E(Tu_t+b)+c$ and study the joint dynamics of $u_t,w_t$. In the first step we update $w_{t+1}$ by
\begin{align*}
    \left( \begin{array}{c} u'_{t+1} \\ w'_{t+1} \end{array} \right) = \left( \begin{array}{cc} E & \\ & E \end{array}\right) \left( \begin{array}{cc} I & 0 \\ T & 0 \end{array} \right) \left( \begin{array}{c} u_{t} \\ w_{t} \end{array} \right) + \left( \begin{array}{c} 0 \\ Eb + c \end{array}\right)
\end{align*}
In the second step we update $u_{t+1}$ either by
\begin{align*}
    \left( \begin{array}{c} u_{t+1} \\ w_{t+1} \end{array} \right) = \left( \begin{array}{cc} E & \\ & E \end{array}\right) \left( \begin{array}{cc} -H & H+I \\ 0 & I \end{array} \right) \left( \begin{array}{c} u'_{t+1} \\ w'_{t+1} \end{array} \right) + \left( \begin{array}{c} c \\ 0 \end{array}\right)
\end{align*}
Or equivalently by
\begin{align*}
    \left( \begin{array}{c} u_{t+1} \\ w_{t+1} \end{array} \right) = \left( \begin{array}{cc} E & \\ & E \end{array}\right) \left( \begin{array}{cc} T-H & H \\ 0 & I \end{array} \right) \left( \begin{array}{c} u'_{t+1} \\ w'_{t+1} \end{array} \right) + \left( \begin{array}{c} Eb + c \\ 0 \end{array}\right)
\end{align*}
We first consider the first case, 
\begin{align*}
    \left( \begin{array}{c} u_{t+1} \\ w_{t+1} \end{array} \right) = \left( \begin{array}{cc} E & \\ & E \end{array}\right) \left( \begin{array}{cc} T-H & 0 \\ H & I \end{array} \right) \left( \begin{array}{cc} E & \\ & E \end{array}\right) \left( \begin{array}{cc} I & 0 \\ T & 0 \end{array} \right) \left( \begin{array}{c} u_{t} \\ w_{t} \end{array} \right) + C
\end{align*}
where $C$ is some vector with no dependence on $(u_t, w_t)$. Therefore to analyze convergence of the system, we observe that 
\begin{align*}
    \left\lVert \left( \begin{array}{cc} E & \\ & E \end{array}\right) \right\rVert_2 &< 1 \\
    \left\lVert \left( \begin{array}{cc} I & 0 \\ T & 0 \end{array} \right) \right\rVert_2^2 &= \sup_{\lVert x_1 \rVert_2^2 + \rVert x_2 \rVert_2^2=1} \left\lVert \left( \begin{array}{cc} I & 0 \\ T & 0 \end{array} \right) \left( \begin{array}{c} x_1 \\ x_2 \end{array} \right) \right\rVert_2^2 \\
    &= \sup_{\lVert x_1 \rVert_2^2 + \rVert x_2 \rVert_2^2=1} \lVert x_1 \rVert_2^2  + \lVert Tx_1 \rVert_2^2 &\leq \sup_{\lVert x_1 \rVert_2^2 + \rVert x_2 \rVert_2^2=1}  \\
    \left\lVert \left( \begin{array}{cc} -H & H+I \\ 0 & I \end{array} \right) \right\rVert &= \max(\rho(-H), 1) = \max(\rho(H), 1)  \\
\end{align*}
Therefore if we have $\rho(H) \leq 1$ then all the above terms have spectral norm $<1$ or $\leq 1$, by triangle inequality we have
\[ \rho \left( \left( \begin{array}{cc} E & \\ & E \end{array}\right) \left( \begin{array}{cc} -H & H+I \\ 0 & I \end{array} \right) \left( \begin{array}{cc} E & \\ & E \end{array}\right) \left( \begin{array}{cc} I & 0 \\ T & 0 \end{array} \right) \right) < 1 \]
which proves that the joint dynamics on $(u_t, w_t)$ converges. Therefore $u_t$ must also converge. Identially we may also prove that the dynamics converge if $\rho(T-H) < 1$. 
\end{proof}


